Eye-Shield: Real-Time Protection of Mobile Device Screen Information from Shoulder Surfing

People use mobile devices ubiquitously for computing, communication, storage, web browsing, and more. As a result, the information accessed and stored within mobile devices, such as financial and health information, text messages, and emails, can often be sensitive. Despite this, people frequently use their mobile devices in public areas, becoming susceptible to a simple yet effective attack, shoulder surfing. Shoulder surfing occurs when a person near a mobile user peeks at the user's mobile device, potentially acquiring passcodes, PINs, browsing behavior, or other personal information. We propose Eye-Shield, a solution to prevent shoulder surfers from accessing or stealing sensitive on-screen information. Eye-Shield is designed to protect all types of on-screen information in real time, without any serious impediment to users' interactions with their mobile devices. Eye-Shield generates images that appear readable at close distances, but appear blurry or pixelated at farther distances and wider angles. It is capable of protecting on-screen information from shoulder surfers, operating in real time, and being minimally intrusive to the intended users. Eye-Shield protects images and text from shoulder surfers by reducing recognition rates to 24.24% and 15.91%. Our implementations of Eye-Shield, with frame rates of 24 FPS for Android and 43 FPS for iOS, effectively work on screen resolutions as high as 1440x3088. Eye-Shield also incurs acceptable memory usage, CPU utilization, and energy overhead. Finally, our MTurk and in-person user studies indicate that Eye-Shield protects on-screen information without a large usability cost for privacy-conscious users.

==> FiguresTex/fig_color_range.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{Figures/colors.pdf}
  \caption{The number (range) of color pairs that \name is 100\% guaranteed to protect for a given RGB color with R set to 168. Note that there are 16,777,216 possible colors in the RGB color space.}
  \label{fig:colors}
\end{figure}


==> FiguresTex/fig_entropy.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Figures/gridsize_entropy_dataset.pdf}
  \caption{}
  \label{fig:entropy_grid}
\end{subfigure}
% \begin{subfigure}{\columnwidth}
%   \centering
%   \includegraphics[width=\columnwidth]{Figures/downscale_entropy_dataset.pdf}
%   \caption{}
%   \label{fig:entropy_downscale}
% \end{subfigure}
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Figures/parameter_entropy_dataset.pdf}
  \caption{}
  \label{fig:entropy_parameter}
\end{subfigure}
\caption{}
\label{fig:entropy}
\end{figure}

==> FiguresTex/fig_examples_gallery.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/0827.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/0842.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/0846.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/0855.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/0859.pdf}
\end{subfigure}
\caption{}
\label{fig:gallery_images_protected}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/1622.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/2322.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/2559.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/2627.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/protected/6278.pdf}
\end{subfigure}
\caption{}
\label{fig:gallery_text_protected}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/0827.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/0842.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/0846.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/0855.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/0859.pdf}
\end{subfigure}
\caption{}
\label{fig:gallery_images}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/1622.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/2322.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/2559.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/2627.pdf}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/unprotected/6278.pdf}
\end{subfigure}
\caption{}
\label{fig:gallery_text}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.49\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/close_protected/0827.pdf}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/close_protected/0855.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/close_protected/0859.pdf}
\end{subfigure}
\caption{}
\label{fig:gallery_images_close}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/close_protected/2559.pdf}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/close_protected/2627.pdf}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/examples/close_protected/6278.pdf}
\end{subfigure}
\caption{}
\label{fig:gallery_text_close}
\end{figure*}


==> FiguresTex/fig_memory.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Figures/cpu_memory.pdf}
  \caption{CPU-Only Memory \\(Desktop)}
  \label{fig:cpu_memory}
\end{subfigure}
\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Figures/gpu_memory.pdf}
  \caption{With-GPU Memory \\(All Platforms)}
  \label{fig:gpu_memory}
\end{subfigure}
\caption{The memory usage scales with the resolution size, reaching up to 40.04MB per frame in the GPU implementation of \name (b). Using only the CPU consumes more memory with each frame (up to 299.95MB).}
\label{fig:memory}
\end{figure}

==> FiguresTex/fig_ssim_original.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Figures/gridsize_similarity_dataset_original.pdf}
  \caption{SSIM scores with different grid sizes.}
  \label{fig:ssim_gridsize_original}
\end{subfigure}
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Figures/parameter_similarity_dataset_original.pdf}
  \caption{SSIM scores with different blurring intensities.}
  \label{fig:ssim_parameter_original}
\end{subfigure}
\caption{SSIM scores for each evaluated dataset while varying different parameters such as grid size, downscaling size, and blurring/pixelation intensity. SSIM scores are computed by comparing the downscaled protected image and blurred/pixelated image}
\label{fig:ssim_original}
\end{figure}

==> FiguresTex/fig_userstudy.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\columnwidth]{Figures/userstudy.pdf}
  \caption{In-person user study setup.}
  \label{fig:userstudy}
\end{figure}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> Source/900_Revisions.tex <==
\newpage
\onecolumn
{\begin{center}
\section*{Major Revision Response}
\end{center}
}
\setcounter{page}{1}
We appreciate the reviewers' thoughtful comments and suggestions for our paper \textbf{Real-Time Protection of Mobile Device Screen Information from Shoulder Surfing}, previously submitted July 2022 to the Summer cycle of \textit{USENIX Security Symposium 2023}. In this revision, we made changes according to both the reviewers' and the shepherd's suggestions. Given the addition of new experiments in this submission, some of the less crucial results appear in the appendix or have been removed. This response letter consists of two sections: a general summary of changes, and the changes made in response to the shepherd's suggestions. ({\em If we were allowed to use an additional space beyond 13 pages, we could include the details given below in the final version of this paper}.)

\subsection*{Summary of Changes}


\begin{enumerate}
    \item Expand the user study as promised: increasing the number of participants with the goal of diversifying the sample (\cref{subsec:method_user_study,subsec:results_usability})
    \begin{enumerate}
        \item We expanded user study to include 15 new in-person participants (for a total of 22 participants). We recruited participants with a wide range of ages (22--63 yo), racial/ethnic backgrounds (African, Hispanic, Asian, White), smartphone usage experience (somewhat proficient -- very proficient), and vision problems (trifocals, dry eye, older participants with worse vision).
        \item The new user study design was kept mostly consistent with the addition of another half hour (total 1 hour, \$20 per participant) to add time for evaluating different angles, including evaluation of a privacy film, and obtaining more in-depth qualitative feedback.
        \item Overall out of 15 participants, only 8 participants indicated they would be uncomfortable with shoulder surfers peeking at their devices. 7 participants indicated they preferred using \name over using a privacy film, 7 participants found an option to set the blurring intensity to be useful, and 6 participants stated that the ability to toggle \name would be helpful. 7 participants stated they would use \name for protecting financial data and PIN entry, and 3 participants said they would use it to protect personal texts and photos.
        \item Participants also indicated that zooming, leaning in, increasing brightness, and using blur instead of pixelation improved the usability of \name as the intended user.
        \item We also observed generational differences in our responses, for example, older participants generally used their phone less in public and found less of a need for \name whereas younger participants were the opposite.
        \item In our user study, one participant suggested that \name may not function as well for other languages, such as those with thinner lines (e.g., Arabic or Chinese). 
        \item The results of our new user study indicate some decline in the interpretability of images for intended users and the usability score. This is attributed to the addition of older participants and 7 participants who were unbothered by shoulder surfing, who did not see a use for \name. However, the updated usability score is still above average.
        \item Since the Amazon Mechanical Turk study was subject to less strict study procedures, we expanded our in-person user study, so that our in-person results could complement and support the findings of our Mechanical Turk study.
    \end{enumerate}

    \item Add a comparison to privacy films (\cref{subsec:privacy_film})
    \begin{enumerate}
        \item We compared the usability and efficacy of privacy films in various settings with \name in our new in-person user study. About half of the participants mentioned they preferred \name to a privacy film, mainly due to its ability to be toggled on and off and its increased protection guarantees. Some participants found the privacy film disorienting and unpleasant to use when not viewing the screen directly. While a physical privacy film is effective in protecting all content from a $\geq 45 \degree$ angle, it is ineffective if the device is in landscape orientation. Additionally, its efficacy is dependent on the relative brightness of the screen compared to the environment lighting. It is also unable to protect any content for $\leq 30 \degree$ angles. However, the privacy film has an advantage over \name in that it can protect against optical zoom as shown in \cref{table:film}.
        \item We also combined both \name and a physical privacy film and found that combining the two protection mechanisms adds increased protection by reducing the visible angle, requiring shoulder surfers to lean over an extra 6 inches to be able to read any content. It also more effectively protects content on screens with 100\% brightness.
    \end{enumerate}

    \item Expand the comparison between HideScreen and Eye-Shield in the paper, as demonstrated in the first section of the author response (\cref{subsec:comparison})
    \begin{enumerate}
        \item We added more comparison details to \cref{subsec:comparison} for \name, \hidescreen, and Zezschwitz \etal. We highlighted several of the differences we discussed in our author response.
    \end{enumerate}

    \item Include the discussion of eye-strain ethical considerations taken during the user study in the paper (\cref{subsec:results_usability,subsec:limitations})
    \begin{enumerate}
        \item In our new user study, only 3 participants stated they experienced eyestrain as the intended user. They noted that it was only minor eyestrain.
        \item We added a discussion of eyestrain and potential long-term effects on vision for prolonged usage of \name. We found that any potential risk of negative impacts with \name is minimized by limiting the activation of \name for sensitive information.
        \item We added a potential method to improve the usability of \name for visually impaired participants in \cref{subsec:limitations}. We also added details for real-world deployment details and integration with accessibility APIs.
    \end{enumerate}

    \item Include the methodological clarifications around lighting/screen brightness, binary recognition, study order, and phone position (\cref{subsec:method_mturk_study,subsec:method_user_study})
    \begin{enumerate}
        \item We added clarifications on the order of settings shown in the user studies and explained that its purpose was to minimize bias.
        \item We discussed how we calculated binary accuracy for the subjective/objective user study answers.
        \item We provided an explanation of the fixed phone positioning and the screen and environment brightness for the in-person study.
    \end{enumerate}

    \item Include a note in the appendix about the downscaling of sample images (\cref{sec:examples})
    \begin{enumerate}
        \item We added a note about quality degradation regarding the Appendix figures.
        \item To save space, we also opted to remove several redundant Appendix figures from the paper and decided to host them on an external website which will be made available in the camera-ready version of the paper.
    \end{enumerate}

    \item Brightness, contrast, and environmental lighting (\cref{subsec:contrast_brightness})
    \begin{enumerate}
        \item We added the results and discussion of screen/environment brightness and contrast to \cref{subsec:contrast_brightness} (as previously discussed in the author response).
    \end{enumerate}

    \item Writing Improvements
    \begin{enumerate}
        \item Removed redundant paragraphs in introduction and conclusion.
        \item Various word choice and clarification changes (e.g., ``indifferent and receptive'').
        \item Added units to \cref{fig:resources} and increased size of \cref{fig:mturk_other}.
        \item Changed OCR and Cloud Vision results to an ECDF plot with proportion rather than a count.
        \item Cleaned up the presentation of several equations, algorithms, and the performance plots.
        \item Moved several equations and tables to the appendix and added captions to Appendix figures.
        \item Removed a redundant figure depicting the user study setup (already covered in \cref{fig:threat_model}) and MTurk response times.
    \end{enumerate}
\end{enumerate}

